Active Perception Applied To Unmanned Aerial Vehicles Through Deep Reinforcement Learning

Unmanned Aerial Vehicles (UAV) have been standing out due to the wide range of applications in which they can be used autonomously. However, they need intelligent systems capable of providing a greater understanding of what they perceive to perform several tasks. They become more challenging in complex environments since there is a need to perceive the environment and act under environmental uncertainties to make a decision. In this context, a system that uses active perception can improve performance by seeking the best next view through the recognition of targets while displacement occurs. This work aims to contribute to the active perception of UAVs by tackling the problem of tracking and recognizing water surface structures to perform a dynamic landing. We show that our system with classical image processing techniques and a simple Deep Reinforcement Learning (Deep-RL) agent is capable of perceiving the environment and dealing with uncertainties without making the use of complex Convolutional Neural Networks (CNN) or Contrastive Learning (CL).

==> backup.tex <==
% \begin{document}



% \maketitle
% \thispagestyle{empty}
% \pagestyle{empty}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{abstract}

% Com o aumento nas áreas de estudo envolvendo veículos autônomos, os veículos áereos não-tripulados vem se destacando devido a grande gama de aplicações nas quais podem ser utilizados. Essa capacidade de atuação implica no crescimento da demanda por sistemas cada vez mais inteligentes, capazes de proporcionar uma maior compreensão do ambiente ao qual o veículo está inserido. E se tratando de ambientes abertos e com grande complexidade, como acontece em terrenos encontrados na natureza, a precisão na atuação do sistema precisa ser ainda maior, o que traz a necessidade de perceber o ambiente com diversas variáveis efetuando uma constante tomada de decisão. Dessa forma um sistema que emprega a percepção ativa em um véiculo atua com diversos sensores trazendo a visão como seu principal coletor de informação, buscando um posicionamento que favoreça o reconhecimento de alvos enquanto ocorre o deslocamento. Nesse contexto, no presente trabalho é proposto uma abordagem para o desenvolvimento da percepção ativa, com o intuito de efetuar o rastreamento e reconhecimento de um alvo na superfície da água para a efetuação do pouso. Assim, buscando uma abordagem foto-realística se utilizou o plugin \textit{AirSim} juntamente com a \textit{Unreal Engine} para o desenvolvimento do método proposto, visando a caracterização da percepção ativa através do aprendizado por reforço profundo. Para isso, a geração da observação do agente é feita através da interpretação do processamento da visão, não necessitando a utilização de redes neurais convolucionais ou aprendizado contrastivo. Levando à obtenção de resultados satisfatórios quanto à política aprendida pelo agente durante os testes desempenhados, possibilitando efetuar o pouso com o alvo disposto em diversas posições e orientações dentro do campo de visão do agente.

% \end{abstract}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{INTRODUCTION}
% Os veículos aéreos não-tripulados (\textit{UAVs}) são um dos tipos de veículos autônomos que vem ganhando cada vez mais espaço devido a versatilidade em suas possíveis aplicações, algumas delas enfrentam as problemáticas que envolvem atuar sobre a água para desempenhar suas respectivas tarefas. Como acontece nas diferentes áreas de monitoramento hidrológico~\cite{velez2021applications}, principalmente em aplicações de sensoriamento remoto~\cite{perumal2017uav}. Problema que surge também nas atuações em missões de busca e salvamento com o reconhecimento de vítimas na superfície da água~\cite{qingqing2020towards}, além do monitoramento da fauna marinha~\cite{gaspar2015model}, da navegação conjunta entre barcos autônomos e \textit{UAVs}~\cite{garberoglio2019coordinated} e do reconhecimento e monitoramento da poluição através da detecção de lixo na superfície marinha~\cite{gonccalves2020mapping}. Os desafios de detectar, rastrear e seguir um alvo estático ou móvel de interesse é um ponto crítico para todas as aplicações. O reconhecimento desses alvos se torna muito mais complexo comparado a atuação sobre terrenos sólidos, tendo em vista que a refletância da luz sofrida pelas ondulações na superfície da água e outras diferentes influências da incidência de luz vem à prejudicar o fluxo óptico capturado nas imagens durante o voo. 

% A necessidade de unir as informações contidas nas imagens e na leitura de outros sensores durante o voo para a tomada de decisão do veículo é muitas vezes um problema complexo, já que as leituras são diretamente afetadas pelo posicionamento atual e posicionamento futuro afetado pela leitura atual. O que traz a demanda de efetuar a movimentação buscando sempre o maior ganho de informação ou a próxima melhor visão (\textit{NBV}), e assim propriamente caracterizando uma percepção ativa~\cite{gemerek2020active}.

% Nesse contexto, se propôs lidar com o problema de atuar sobre água efetuando o rastreamento e o deslocamento percebendo ativamente o ambiente para a conclusão do pouso em uma base disposta na superfície da água. Dada a natureza do problema, surgiu a necessidade da utilização do plugin \textit{AirSim}, visando a utilização dos ambientes foto-realísticos da \textit{Unreal Engine}. Que também colaborou para o uso da abordagem de aprendizado por reforço profundo (\textit{Deep-RL}), através do suporte fornecido a esse tipo de aprendizado no ambiente da engine. Com a análise sobre a abordagem de \textit{Deep-RL} foi possível constatar que os algoritmos tendem a não convergir com espaços de observação muito grandes, onde o uso de imagens para a observação do agente corresponde a tal problema. Para tornar possível que o algoritmo então convirja, propõe-se a maior contribuição no contexto do desenvolvimento do presente trabalho. De modo que para simplificar o espaço de observação do agente é feita a interpretação do processamento da visão funcionando com o mesmo propósito de um \textit{Variational Autoencoder}, buscando reescrever os dados da imagem bruta nas distâncias em \textit{pixels} referente aos eixos $x$ e $y$. Assim, levando o algoritmo a convergir sem o uso de redes neurais convolucionais ou aprendizado contrastivo mesmo dentro de um ambiente extremamente realístico.


% \section{RELATED WORKS}
% O conceito de um observador ativo é pré-estabelecido por~\cite{bajcsy2018revisiting} quanto por~\cite{gemerek2020active}, quando o mesmo desempenha algum tipo de atividade cuja finalidade é controlar os parâmetros geométricos do aparelho sensorial. Tendo como objetivo da atividade, manipular as restrições subjacentes aos fenômenos observados para melhorar a qualidade dos resultados perceptivos. Ou seja, a constituição da percepção ativa ocorre quando o observador altera sua posição e/ou a posição dos seus sensores a fim de obter a maior quantidade de informação sobre o ambiente em que está inserido. Também definida como a união do controle inteligente ou controle ativo e da percepção visual ou visão ativa.

% %Esse conceito é muito explorado em aplicações que buscam de alguma forma reconstruir o ambiente, onde a estimativa do \textit{NBV} é um pouco mais crítica, como acontece em~\cite{kong2020active} onde é proposto um método para modelar geometrias com formas relativamente regulares e em~\cite{nishimura2018active} ondem se propõe decodificar mensagens através de um UAV receptor empregadas por outro UAV chamado de remetente. Em situações mais próximas de aplicações no mundo real ocorrem algumas adaptações, principalmente em relação ao posicionamento do sensor visual, mas o principio ainda é o mesmo como acontece em~\cite{liu2012fast} buscando o reconhecimento de cabos de energia, com o intuito de utilizar \textit{UAVs} para manutenção, na atuação em vigilância proposta em~\cite{danelljan2014low} buscando a detecção e rastreamento de pessoas em condições de voo totalmente autônomo mantendo o veículo a uma certa distância de uma pessoa e em~\cite{czuni2018lightweight} com a detecção de objetos durante o voo.%

% Esse conceito é muito explorado em aplicações que buscam de alguma forma reconstruir o ambiente ou a cena em si, onde a estimativa do \textit{NBV} é um pouco mais crítica em termos de otimização, como acontece em~\cite{kong2020active} e em~\cite{nishimura2018active}. Em situações mais próximas de aplicações no mundo real ocorrem algumas adaptações, principalmente em relação ao posicionamento do sensor visual, mas o principio ainda é o mesmo como acontece em~\cite{liu2012fast},~\cite{danelljan2014low} e~\cite{czuni2018lightweight}. Avaliando a problemática de sobrevoar e efetuar a detecção de alvos na superfície da água com o deslocamento até eles, tendo a percepção visual como protagonista, se tem principalmente abordagens envolvendo o reconhecimento e diferenciação de terreno~\cite{pombeiro2015water} e ~\cite{matos2018uav}, e poucos trabalhos buscando por alvos específicos na superfície como em~\cite{qingqing2020towards} e ~\cite{singh2020simulating}.   

% Com a analise dos trabalhos encontrados, foi possível perceber o uso de diversos algoritmos para estimar e efetuar o posicionamento do UAV. A fim de aproveitar o suporte do \textit{AirSim} e o amplo conceito de percepção ativa, se buscou por trabalhos que se utilizam de algoritmos de \textit{Deep-RL} focados em deslocamento com base na percepção visual. Assim foram analisados trabalhos como de \cite{sampedro2019fully} onde foi proposto o uso do algoritmo de \textit{Deep-RL} denominado Gradientes de Política Determinística Profundos (\textit{DDPG}) aplicado a tarefa de busca e resgate em um ambiente fechado. Esse mesmo algoritmo foi utilizado por \cite{kang2019generalization}, tendo o foco na atuação de reconhecer e desviar de alvos e por \cite{rodriguez2019deep} onde foi proposto o uso do \textit{DDPG} para a efetuação do pouso em uma base móvel. Os 3 trabalhos citados fazem uso tanto da utilização de dados simulados (Gazebo) quanto de dados reais, além da validação do método em ambos os ambientes. Assim tendo em vista a abordagem do trabalho apresentado por \cite{rodriguez2019deep} onde se tem como foco a tarefa de pouso com alta acurácia nos resultados, é utilizado como principal referência para a implementação do sistema proposto.  

% \section{ENVIRONMENT CONSTRUCTION}
% A escolha do plugin \textit{AirSim} foi feita buscando melhorar a qualidade do ambiente em que o UAV irá atuar, já que foi desenvolvido pela \textit{Microsoft} visando os custos de desenvolver e testar algoritmos para veículos autônomos no mundo real. O \textit{AirSim} fornece uma interface para definir o veículo como um corpo rígido que pode ter um número arbitrário de atuadores gerando forças e torques. A geração de todos os modelos matemáticos voltados a física do veículo e seus sensores foram estimados baseados em veículos reais, trazendo um resultado bem próximo entre a simulação e a atuação de um UAV real como é descrito por~\cite{shah2018airsim}. O \textit{AirSim} foi desenvolvido para a \textit{Unreal Engine}(https://www.unrealengine.com/en-US/), sendo ela desenvolvida é mantida pela desenvolvedora de jogos \textit{Epic Games}, que é responsável pelo desenvolvimento de diversos jogos famosos no mercado. A grande qualidade apresentada nos gráficos disponíveis nos motores fornecidos pela engine vem trazendo novos horizontes para sua utilização, onde na sua própria plataforma é chamado de "modo sério" o uso voltado ao gênero simulação. Assim o uso de simulação para veículos reais vem crescendo, tendo implicações como simuladores de voo e de direção onde a similaridade com um ambiente real é de altíssima importância.

% No trabalho foi aderida a versão 4.25 do motor da engine utilizando o ambiente denominado \textit{Landscape Mountain} fornecido gratuitamente no mercado de desenvolvimento da \textit{engine}, juntamente com uma superfície hídrica (https://free3d.com/3d-model/ocan-1761.html) e um bote de pesca (https://free3d.com/3d-model/boat-6219.html), demonstrados na Fig~\ref{fig_ambiente_unreal}. O veículo utilizado pelo \textit{AirSim} é um modelo \textit{AirDrone} com uma grande diversidade de possíveis sensores podendo ser agregados a sua estrutura, como \textit{GPS}, Lidar, magnetômetro, barômetro e mais de uma câmera com alguns formatos de imagem além do convencional \textit{RGB}. Essas configurações podem ser todas modificadas através de um arquivo \textit{.xml} com os respectivos parâmetros de cada sensor. Assim no presente trabalho são usados apenas o barômetro e uma câmera com a captura convencional alocada no centro do veículo direcionada para baixo da mesma forma que em~\cite{liu2012fast}.

% \begin{figure}[thpb]
%       \centering
%       \includegraphics[scale=0.13]{imgs/fig_ambiente_unreal.png}
%       \caption{Inductance of oscillation winding on amorphous magnetic core versus DC bias magnetic field}
%       \label{fig_ambiente_unreal}
% \end{figure}

% \section{PERCEPTION IMPLEMENTATION}
% Foi criado um pacote ROS (https://www.ros.org/) denominado \textit{"active\_perception"}, onde são implementados dois nodos buscando respectivamente a detecção e o pouso. O nodo encarregado pela detecção é denominado \textit{"cam\_listener"}, responsável por fazer a leitura da câmera e publicar no tópico \textit{"vision"} a mensagem com as distâncias do alvo em pixels nos eixos $x$ e $y$. E o nodo \textit{land} responsável pelas decisões de deslocamento e efetuar propriamente o pouso com base nas leituras do tópico \textit{"vision"}. 
% \subsection{Detection}
% Para efetuar a detecção do bote a busca é dividida em duas etapas, primeiro analisando o reflexo da luz na superfície da água e em seguida a busca pelo bote. Para efetuar a detecção da luz, a imagem original capturada pela câmera é convertida para escala de cinza e então aplicado o Desfoque Gaussiano (1) avaliando a variância dos pixels em ambas as direções, e salvando o primeiro frame processado. A partir do segundo frame é analisado o fluxo óptico na imagem através do método Lucas-Kanade~\cite{LK}, onde é feita a comparação no deslocamento dos pixels com base na distância dos vizinhos buscando mudanças tendo os parâmetros adaptados para o reflexo da luz. 
% $$
% G(x, y) = \frac{1}{2\pi\sigma^2}\dot{e}^{\frac{x^2 + y^2}{2\sigma^2}} \eqno{(1)}
% $$

% Com base nos pontos em que foram encontradas modificações é calculado o centroide da região gerada pelos pontos, e então criada a partir dele uma máscara a ser aplicada sobre a imagem em escala de cinza como mostra a Fig~\ref{fig_filters} (a). Com ela é feita a aplicação do algoritmo de \textit{Canny} (2) para detectar possíveis bordas através da analise tanto da largura quanto do comprimento da imagem. 

% $$
%  G'(x, y) = \frac{\sqrt{x^2 + y^2}}{2\pi\sigma^4}\dot{e}^{\frac{x^2 + y^2}{2\sigma^2}} \eqno{(2)}
% $$

% Por fim é aplicada uma transformação morfológica na imagem sendo uma dilatação seguida por erosão buscando pelo contorno com a maior área, tendo como resultado a Fig~\ref{fig_filters} (b) e através do cálculo do centro do contorno são calculadas as distâncias em \textit{pixels} do alvo nos eixos $x$ e $y$ e publicadas no tópico \textit{"$\backslash$vision"}. Assim visualmente o resultado das duas analises acontece como é demonstrado na Fig~\ref{fig_filters} (c).

% \begin{figure}[htb]
%     \begin{minipage}[c][0.75\width]{0.235\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{imgs/fig_ambiente_unreal.png}
%           \textbf{a)}
% 	\end{minipage}
%     \begin{minipage}[c][0.75\width]{0.235\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{imgs/fig_ambiente_unreal.png}
%           \textbf{b)}
% 	\end{minipage} \vfill
%     \begin{minipage}[c][0.75\width]{0.235\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{imgs/fig_ambiente_unreal.png}
%           \textbf{c)}
% 	\end{minipage}
%  \caption{Inductance of oscillation winding on amorphous
%       magnetic core versus DC bias magnetic field}
%       \label{fig_filters}
% \end{figure}


% \subsection{Land}
% No algoritmo \textit{DDPG}~\cite{ddpg} o ator mapeia diretamente estados para ações em vez de gerar a distribuição de probabilidade em um espaço de ação discreto como é originalmente feito por outros algoritmos do mesmo modelo. As outras duas redes são redes de destino, sendo elas cópias com atraso de tempo de suas redes originais que rastreiam suavemente as redes aprendidas. O uso das redes de valor-alvo melhora muito a estabilidade no aprendizado, já que as equações de atualização das redes principais são dependentes dos valores calculados por elas mesmas tornando-as propensas a divergências. O \textit{DDPG} também usa um \textit{buffer} de repetição para amostrar a experiência e atualizar os parâmetros da rede neural. No aprendizado por reforço para espaços de ação discretos, a exploração é feita por meio da seleção probabilística de uma ação aleatória. Para espaços de ação contínuos, a exploração é feita adicionando ruído à própria ação, como foi empregado no trabalho, podendo também ser utilizado no estado. Um dos métodos mais utilizados é o Processo \textit{Ornstein-Uhlenbeck}~\cite{OU} para adicionar ruído à saída, onde é correlacionado com o ruído anterior de modo a evitar que o ruído cancele a dinâmica geral criada pelo Ator. 

% Para a adaptação da proposta desenvolvida por \cite{rodriguez2019deep} visando a simplificação no desenvolvimento, é utilizado o módulo na linguagem Python para lidar com redes neurais Pytorch (https://pytorch.org/). Sendo assim feita a adaptação de um modelo para outro utilizando a mesma composição para a estrutura das redes como demonstrado na \ref{fig_redes}, tendo sido modificadas as dimensões das camadas ocultas para 300 e 200 unidades. 

% \begin{figure}[thpb]
%       \centering
%       \includegraphics[scale=0.13]{imgs/fig_ambiente_unreal.png}
%       \caption{Inductance of oscillation winding on amorphous magnetic core versus DC bias magnetic field}
%       \label{fig_ambiente_unreal}
% \end{figure}

% Para o espaço de ação se manteve o mesmo princípio, utilizando apenas as velocidades lineares em $x$ e $y$ com a velocidade em $z$ sendo constante. Já no espaço de estados é passado para o agente as distâncias $x$ e $y$ em pixels lidas através da publicação no tópico \textit{"vision"} feita com o processamento da imagem. Para a implicação das ações tendo em vista que a saída da rede Ator varia entre -1 e 1 por ser uma função tangente hiperbólica, após a incrementação do ruído \textit{Ornstein-Uhlenbeck} é feita a normalização entre -0.25m/s e 0.25m/s para serem passados como velocidades ao controle de baixo nível do veículo. Por fim, foi elaborada uma função de recompensa onde $d_t$ é obtido através do módulo das distâncias $x$ e $y$ em pixels (4), resultando na função (5) que avalia as distâncias para enviar a recompensa adequada para o agente. As recompensas são dadas com base na conclusão do pouso como maior recompensa, uma recompensa mínima para diminuição da distância, nenhuma recompensa para um aumento na distância até o alvo e por fim uma recompensa negativa para quando o alvo é perdido de vista.

% $$
%  d_t = \sqrt{{d}_{x}^{2} + {d}_{y}^{2}} \eqno{(4)}
% $$

% $$
% r(s_t, a_t) = 
%               \begin{cases}
%                 250          & \text{if } d_t <= 10\\
%                 0,1          & \text{if } d_t < d_{t-1}\\
%                 0            & \text{if } d_t >= d_{t-1}\\
%                 -10          & \text{if } d_t = 1000000.0\\
                
%             \end{cases} \eqno{(5)}
% $$

% A estrutura do sistema final caracterizando a percepção ativa é apresentado na Fig~\ref{fig_diagrama_sistema}, levando então para a analise dos resultados obtidos pelo algoritmo apresentados na próxima seção.

% \begin{figure}[thpb]
%       \centering
%       \includegraphics[scale=0.13]{imgs/fig_ambiente_unreal.png}
%       \caption{Inductance of oscillation winding on amorphous magnetic core versus DC bias magnetic field}
%       \label{fig_diagrama_sistema}
% \end{figure}

% \section{Results}
% \subsection{Experimental Setup}
% Para a obtenção dos resultados e propriamente o desenvolvimento do trabalho foi utilizado o sistema operacional \textit{Ubuntu 20.04 LTS}, com a linguagem \textit{C++} utilizada para o processamento de imagem na versão $9.3.0$ e a linguagem \textit{Python} utilizada para o treinamento do agente através do módulo \textit{Pytorch} na versão $3.8.10$. Tendo em vista a possibilidade da aceleração por \textit{hardware} (\textit{GPU}) através da \textit{Unreal Engine} e também sua demanda em processamento gráfico, foi utilizada uma \textit{GPU} do modelo \textit{RTX - 2080 Ti} possuindo a versão $10.1$ de suporte ao processamento paralelo CUDA. Sendo utilizada para o processamento principal uma \textit{CPU} \textit{Intel Core i7-7700k}, contando também com 32 \textit{GB} de memória \textit{RAM}.

% \subsection{Training}
% Para a fase de treinamento, a situação a qual foi imposta ao agente através do ambiente consiste na analise da distância até o bote através da função de recompensa demonstrada anteriormente em (5). Assim caso o agente venha a obter a recompensa máxima dentro de um episódio, o ambiente é reiniciado e o episódio então concluído. Já para as demais recompensas como o caso de o agente perder o bote de vista e obter uma recompensa negativa, somente a simulação é reiniciada e nas recompensas constantes não há reinicio da simulação, apenas a atribuição da recompensa. São definidos os parâmetros do agente baseados nos parâmetros utilizados por \cite{rodriguez2019deep}, sendo o espaço de estados ($4$), o espaço de ação ($2$), o buffer de repetição ($50000$), o fator gama ($0,99$), a taxa de aprendizagem do ator ($1e^{-4}$), a taxa de aprendizagem do crítico ($1e^{-3}$) e o fator de atualização para com as redes alvo ($1e^{-3}$). Assim foi definido a utilização de $1000$ passos dentro de cada episódio, levando a utilização de lotes de $512$ amostras a serem salvas na memória. Foram utilizados $1800$ episódios equivalentes a mais de 24 horas de tempo real, buscando uma política capaz de efetuar o pouso. Na primeira fase do treinamento um alvo é disposto em uma única posição posição, sendo ilustrada pela \ref{fig_treino}, e na segunda com posições variando de forma aleatória caso houvesse a efetuação do pouso. Com a analise dos resultados referentes a parte final foi percebida uma melhora significativa na generalização política aprendida pelo agente, levando a conclusão de que o aprendizado havia sido efetuado. As figuras \ref{fig_treino_r} (a) e \ref{fig_treino_r} (b) ilustram as médias móveis das recompensas, utilizadas para suavizar as discrepâncias, sendo coletadas das duas fases de treinamento. 

% \begin{figure}[thpb]
%       \centering
%       \includegraphics[scale=0.13]{imgs/fig_ambiente_unreal.png}
%       \caption{Inductance of oscillation winding on amorphous magnetic core versus DC bias magnetic field}
%       \label{fig_treino}
% \end{figure}
% \begin{figure}[htb]
%     \begin{minipage}[c][0.75\width]{0.235\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{imgs/fig_ambiente_unreal.png}
%           \textbf{a)}
% 	\end{minipage}
%     \begin{minipage}[c][0.75\width]{0.235\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{imgs/fig_ambiente_unreal.png}
%           \textbf{b)}
% 	\end{minipage} \vfill
%  \caption{Inductance of oscillation winding on amorphous
%       magnetic core versus DC bias magnetic field}
%       \label{fig_treino_r}
% \end{figure}

% Durante o período de treinamento foi possível avaliar que o agente aprendeu a desenvolver trajetórias de forma a se colocar em posições semelhantes ao posicionamento representado pela Fig~\ref{fig_treino_trj} (a) e Fig~\ref{fig_treino_trj} (b), sendo uma consequência da implicação simultânea das velocidades a cada passo, sendo o resultado da busca pelo maior acúmulo de recompensa visando as recompensas por redução da distância e também pela efetuação do pouso. Aprendeu também a se ajustar à deformação ocorrida no contorno pelo efeito da luz, que em determinados ângulos tomados e também pelas guinadas vieram a acontecer. Foi possível analisar também, que o agente generalizou a política de forma a se posicionar colocando o alvo sempre no topo superior direito da imagem com um angulo próximo a 45°, levando a posições críticas no ponto $(0,0)$ da câmera alcançado nos períodos de treino com posições aleatórias, onde a trajetória definida pra o deslocamento até o ponto fez com que fosse necessária a perda da vista do alvo para a movimentação até tal região.
% \begin{figure}[htb]
%     \begin{minipage}[c][0.75\width]{0.235\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{imgs/fig_ambiente_unreal.png}
%           \textbf{a)}
% 	\end{minipage}
%     \begin{minipage}[c][0.75\width]{0.235\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{imgs/fig_ambiente_unreal.png}
%           \textbf{b)}
% 	\end{minipage} \vfill
%  \caption{Inductance of oscillation winding on amorphous
%       magnetic core versus DC bias magnetic field}
%       \label{fig_treino_trj}
% \end{figure}

% Para a estruturação dos gráficos foi feita a coleta do episódio, do tempo e recompensa obtidos ao longo do teste. Dessa forma, foram demonstradas as recompensas máximas obtidas nos testes onde o pouso foi efetuado . E tanto para os casos críticos como para os outros em que o objetivo do agente não foi concluído se utilizando dos $10$ episódios, foi aplicado o valor médio da recompensa obtida durante o determinado teste. Para o gráfico da relação de tempo foi utilizado o tempo máximo de cada teste. Se utilizando tanto para os casos de não convergência quanto para os de convergência, o tempo total para conclusão do teste. 

% \subsection{Assessment of the policy learned}
% Para validar a política desenvolvida pelo agente, foram utilizados parâmetros similares aos do treinamento. Tendo variado apenas na quantidade de passos por episódio, onde foi aumentado até $2000$ para lidar com trajetórias longas. E também o posicionamento do bote em relação ao UAV, onde foram utilizadas posições e orientações aleatórias dentro do campo de visão da câmera. Assim as posições do bote eram alteradas por até $4m$ da posição do UAV nos eixos $x$ e $y$, podendo variar tanto no sentido positivo quanto negativo de cada eixo. Para avaliação da qualidade da política foram desempenhados $100$ testes com posições aleatórias com o intervalo descrito, sendo definido um limite de $10$ episódios para que seja efetuado propriamente o pouso. Assim  foram analisadas as recompensas obtidas pelo agente durante cada teste efetuado e também o tempo necessário para a conclusão do mesmo. Nas figuras Fig~\ref{fig_teste} (a) e \ref{fig_teste}(b) são apresentados respectivamente as recompensas e o tempo real para efetuação do teste.
% \begin{figure}[htb]
%     \begin{minipage}[c][0.75\width]{0.235\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{imgs/fig_ambiente_unreal.png}
%           \textbf{a)}
% 	\end{minipage}
%     \begin{minipage}[c][0.75\width]{0.235\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{imgs/fig_ambiente_unreal.png}
%           \textbf{b)}
% 	\end{minipage} \vfill
%  \caption{Inductance of oscillation winding on amorphous
%       magnetic core versus DC bias magnetic field}
%       \label{fig_teste}
% \end{figure}

% A representação dos gráficos mostra que na grande maioria das vezes o agente conseguiu efetuar o pouso, de forma que as piores recompensas caracterizam a problemática gerada pela perda frequente do alvo. No período de treinamento se pôde avaliar tal fator e durante os testes se comprovou, ressaltando o problema encontrado para efetuar o pouso em alvos próximos ao ponto $(0,0)$ da câmera. De modo que data a trajetória generalizada pela política para o deslocamento até o alvo, o mesmo era perdido de vista nesses casos. A não efetuação do pouso em outras situações não tão críticas, trazem uma grande discrepância com relação aos casos críticos. Porém com relação ao tempo de execução, a maior parte dos casos de não convergência desempenharam um resultado similar de modo que precisaram dos $10$ episódios para conclusão do teste. Analisando os casos em que foi possível efetuar efetivamente o pouso como mostrado na Fig~\ref{fig_teste_p} (a), \ref{fig_teste_p} (b) \ref{fig_teste_p} (c) e \ref{fig_teste_p} (d), o agente necessitou de um tempo médio equivalente a $30$ segundos para concluir a tarefa e então alcançar a maior recompensa. 

% \begin{figure}[htb]
%     \begin{minipage}[c][0.75\width]{0.235\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{imgs/fig_ambiente_unreal.png}
%           \textbf{a)}
% 	\end{minipage}
%     \begin{minipage}[c][0.75\width]{0.235\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{imgs/fig_ambiente_unreal.png}
%           \textbf{b)}
% 	\end{minipage} 
%     \begin{minipage}[c][0.75\width]{0.235\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{imgs/fig_ambiente_unreal.png}
%           \textbf{a)}
% 	\end{minipage}
%     \begin{minipage}[c][0.75\width]{0.235\textwidth}
% 	   \centering
% 	   \includegraphics[width=\textwidth]{imgs/fig_ambiente_unreal.png}
%           \textbf{b)}
% 	\end{minipage} \vfill
%  \caption{Inductance of oscillation winding on amorphous
%       magnetic core versus DC bias magnetic field}
%       \label{fig_teste_p}
% \end{figure}

% Na Tabela~\ref{table_teste_ac} são apresentados os percentuais relativos e absolutos referentes ao número de episódios necessários para a conclusão do pouso e um percentual de $0$ para os testes em que a tarefa não foi efetuada. Podendo se concluir que o modelo desenvolveu uma precisão equivalente a $85\%$.
% \begin{table}[h]
% \caption{An Example of a Table}
% \label{table_teste_ac}
% \begin{center}
% \begin{tabular}{|c|c|c|}
% \hline
% Episodes Number & Relative Percentage & Absolute Percentage\\
% \hline
% $0$ & $0\%$ & $15\%$\\
% \hline
% $1$ & $100\%$ & $75\%$\\
% \hline
% $2$ & $50\%$ & $2\%$\\
% \hline
% $3$ & $33.33\%$ & $2\%$\\
% \hline
% $4$ & $25\%$ & $1\%$\\
% \hline
% $6$ & $16.66\%$ & $1\%$\\
% \hline

% \end{tabular}
% \end{center}
% \end{table}
% \section{CONCLUSIONS}
% Foi possível analisar que o processamento da imagem através da extração de características, se mostra funcional como meio de alimentar algoritmos de \textit{Deep-RL} para a efetuação de tarefas percebendo ativamente o ambiente, tendo em vista que determinados ruídos gerados pelo efeito da luz afetaram pouco ou quase nada no aprendizado com a abordagem utilizada, acarretando em duas principais contribuições. 
% \begin{itemize}
%     \item Simulação realística através do plugin \textit{AirSim} com a aplicação do algoritmo de \textit{Deep-RL} \textit{Deep Deterministic Policy Gradients - DDPG}.
%     \item Processamento da percepção visual para o uso como um \textit{encoder} a fim de solucionar o problema de espaço de observações com muitos dados.
% \end{itemize}

% \addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
%                                   % on the last page of the document manually. It shortens
%                                   % the textheight of the last page by a suitable amount.
%                                   % This command does not take effect until the next page
%                                   % so it should come on the page before the last. Make
%                                   % sure that you do not shorten the textheight too much.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section*{APPENDIX}

% Appendixes should appear before the acknowledgment.

% \section*{ACKNOWLEDGMENT}

% The preferred spelling of the word ÒacknowledgmentÓ in America is without an ÒeÓ after the ÒgÓ. Avoid the stilted expression, ÒOne of us (R. B. G.) thanks . . .Ó  Instead, try ÒR. B. G. thanksÓ. Put sponsor acknowledgments in the unnumbered footnote on the first page.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.


% \bibliographystyle{./bibliography/IEEEtran}
% \bibliography{./bibliography/IEEEabrv,./bibliography/IEEEexample}


% % % \begin{thebibliography}{99}

% % % \bibitem{veles_nicolas} Vélez-Nicolás, Mercedes, et al. "Applications of unmanned aerial systems (UASs) in hydrology: A review." Remote Sensing 13.7 (2021): 1359.
% % % \bibitem{LK} B. Lucas e T. Kanade, “An Iterative Image Registration Technique with
% % % an Application to Stereo Vision (IJCAI)”, vol. 81, abr. de 1981.
% % % \bibitem{OU} Uhlenbeck, George E., and Leonard S. Ornstein. "On the theory of the Brownian motion." Physical review 36.5 (1930): 823.
% % % \bibitem{ddpg} Silver, David, et al. "Deterministic policy gradient algorithms." International conference on machine learning. PMLR, 2014.
% % % \bibitem{c5} E. H. Miller, ÒA note on reflector arrays (Periodical styleÑAccepted for publication),Ó IEEE Trans. Antennas Propagat., to be publised.
% % % \bibitem{c6} J. Wang, ÒFundamentals of erbium-doped fiber amplifiers arrays (Periodical styleÑSubmitted for publication),Ó IEEE J. Quantum Electron., submitted for publication.
% % % \bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
% % % \bibitem{c8} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ÒElectron spectroscopy studies on magneto-optical media and plastic substrate interfaces(Translation Journals style),Ó IEEE Transl. J. Magn.Jpn., vol. 2, Aug. 1987, pp. 740Ð741 [Dig. 9th Annu. Conf. Magnetics Japan, 1982, p. 301].
% % % \bibitem{c9} M. Young, The Techincal Writers Handbook.  Mill Valley, CA: University Science, 1989.
% % % \bibitem{c10} J. U. Duncombe, ÒInfrared navigationÑPart I: An assessment of feasibility (Periodical style),Ó IEEE Trans. Electron Devices, vol. ED-11, pp. 34Ð39, Jan. 1959.
% % % \bibitem{c11} S. Chen, B. Mulgrew, and P. M. Grant, ÒA clustering technique for digital communications channel equalization using radial basis function networks,Ó IEEE Trans. Neural Networks, vol. 4, pp. 570Ð578, July 1993.
% % % \bibitem{c12} R. W. Lucky, ÒAutomatic equalization for digital communication,Ó Bell Syst. Tech. J., vol. 44, no. 4, pp. 547Ð588, Apr. 1965.
% % % \bibitem{c13} S. P. Bingulac, ÒOn the compatibility of adaptive controllers (Published Conference Proceedings style),Ó in Proc. 4th Annu. Allerton Conf. Circuits and Systems Theory, New York, 1994, pp. 8Ð16.
% % % \bibitem{c14} G. R. Faulhaber, ÒDesign of service systems with priority reservation,Ó in Conf. Rec. 1995 IEEE Int. Conf. Communications, pp. 3Ð8.
% % % \bibitem{c15} W. D. Doyle, ÒMagnetization reversal in films with biaxial anisotropy,Ó in 1987 Proc. INTERMAG Conf., pp. 2.2-1Ð2.2-6.
% % % \bibitem{c16} G. W. Juette and L. E. Zeffanella, ÒRadio noise currents n short sections on bundle conductors (Presented Conference Paper style),Ó presented at the IEEE Summer power Meeting, Dallas, TX, June 22Ð27, 1990, Paper 90 SM 690-0 PWRS.
% % % \bibitem{c17} J. G. Kreifeldt, ÒAn analysis of surface-detected EMG as an amplitude-modulated noise,Ó presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
% % % \bibitem{c18} J. Williams, ÒNarrow-band analyzer (Thesis or Dissertation style),Ó Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
% % % \bibitem{c19} N. Kawasaki, ÒParametric study of thermal and chemical nonequilibrium nozzle flow,Ó M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
% % % \bibitem{c20} J. P. Wilkinson, ÒNonlinear resonant circuit devices (Patent style),Ó U.S. Patent 3 624 12, July 16, 1990. 






% % \end{thebibliography}




% \end{document}

==> sections/5_discussion.tex <==
\section{Discussion}
\label{discussion}

% REESCREVER, FALAR QUE TD3 E SAC FICARAM MELHOR QUEDDPG E BUG2. FALAR SEMELHANTE AO QUE FOI FEITO NO PAPER DO JINT 

The evaluation shows an overall increase of performance in the navigation through both environments. It is possible to see that our approaches achieves a consistent performance of 100 successfully air-to-water navigation trials with also a consistent navigation time ($14.55 \pm 0.87$ and $11.19 \pm 2.86$). In this same scenario, the stochastic performed a little worse in the air-to-water navigation but outperformed the deterministic approach in the water-to-air navigation. 
In the second scenario, we can see more clearly that a double-critic-based approach with an RNN structure also has a better ability to learn and generalize the environment, including the obstacles and the medium transition. While the state-of-the-art approaches with a MLP structure were not capable to perform the task, our approaches presented once again a consistent performance especially in air-to-water navigation. Our approaches showed an excellent ability to learn the tasks and the environmental difficulties, not only the scenario itself. That was further addressed in our additional evaluation with agents trained in the first environment only, both first and second environments and second environment only. Overall, we can conclude that double critic approaches with recurrent neural networks present a consistent ability to learn through scenarios and environments and to generalize between them. Also, our approaches outperformed the BBA algorithm 
% \cbox{BUG2 algorithm - CHamaria de behaviour-based algorithm ou algo assim} 
in the rate of successful trials and average time in almost all situations.

It is important to mention that these approaches are extensively evaluated in a realistic simulation, including control issues and disturbances such as wind. Thus, the results indicate that our approach may achieve real-world application if the correct data from the sensing and the relative localization are correctly ensured. Finally, it is also possible to analyze that these new RNN-based approaches provided a more consistent average course of actions throughout the environments.
% We can see in Fig.~\ref{fig:cmd} a decrease in the action's standard deviation when compared with the action's standard deviation of the state-of-the-art~\cite{bedin2021deep}. 

% The extensive validation of our proposed reveals a proper behavior for both agents in both environments. The agents were able to learn environmental difficulties, realize the medium transition, and generalize enough to perform the mapless navigation through air and water. Besides that, our agents also learned to bypass obstacles to arrive at a target and managed to outperform a traditional algorithm. We have validated two powerful approaches, which managed to understand the complex behaviors in realistic simulation and that can be used in the real world if guarantying range findings and relative localization data. 

% Specifically, we can also observe that our deterministic approach performed considerably better than our 3DNDRL-S approach in the first and simpler scenario with just simulated wind and a water tank. However, in the second scenario with simulated drilling risers, we can observe based on the results of Table \ref{table:mean_std} and Figs. \ref{fig:traj_nav_1} and \ref{fig:traj_nav_2} that the better exploration policy of the 3DNDRL-S approach made it have a similar or even better performance than our deterministic algorithm. Finally, it is interesting to notice that, besides the fact that our two approaches have fundamental differences in its implementation, the actions generated by each of them at each step of testing when averaged 100 times are quite similar, manly in the second and more complex scenario. We can observe this robustness and consistency in Fig. \ref{fig:cmd}.


